KL Divergence Estimation with Multi-group Attribution

Estimating the Kullback-Leibler (KL) divergence between two distributions given samples from them is well-studied in machine learning and information theory. Motivated by considerations of multi-group fairness, we seek KL divergence estimates that accurately reflect the contributions of sub-populations to the overall divergence. We model the sub-populations coming from a rich (possibly infinite) family $\mathcal{C}$ of overlapping subsets of the domain. We propose the notion of multi-group attribution for $\mathcal{C}$, which requires that the estimated divergence conditioned on every sub-population in $\mathcal{C}$ satisfies some natural accuracy and fairness desiderata, such as ensuring that sub-populations where the model predicts significant divergence do diverge significantly in the two distributions. Our main technical contribution is to show that multi-group attribution can be derived from the recently introduced notion of multi-calibration for importance weights [HKRR18, GRSW21]. We provide experimental evidence to support our theoretical results, and show that multi-group attribution provides better KL divergence estimates when conditioned on sub-populations than other popular algorithms.

==> app-mcab.tex <==
\section{Proofs}
\label{app:mcab}



\subsection{Proofs from Section \ref{sec:intro}}

\begin{proof}[Proof of Lemma \ref{lem:chain-rule}]
We have
\begin{align*}
    \KL{R}{P} &= \E_R\logf{R(x)}{P(x)} \\
    &= R(C)\E_{R|_C}\logf{R(x)}{P(x)} + R(\bar{C})\E_{R|_{\bar{C}}} \logf{R(x)}{P(x)}\\
    & = R(C)\E_{R|_C}\logf{R|_C(x)R(C)}{P|_C(x)P(C)} + R(\bar{C})\E_{R|_{\bar{C}}}\logf{R|_{\bar{C}}(x)R(\bar{C})}{P|_{\bar{C}}(x)P(\bar{C})} \\
    &= R(C)\E_{R|_C}\logf{R|_C(x)}{P|_C(x)} + 
R(\bar{C})\E_{R|_{\bar{C}}}\logf{R|_{\bar{C}}(x)}{P|_{\bar{C}}(x)}\\
& + R(C)\E_{R|_C}\logf{R(C)}{P(C)} +  R(\bar{C})\logf{R(\bar{C})}{P(\bar{C})}\\
&= R(C)\KL{R|_C}{P|_C} + R(\bar{C})\KL{R|_{\bar{C}}}{P|_{\bar{C}}} + \d(R(C), P(C)).
\end{align*}

\end{proof}

The following Lemma proves that distinguishing whether the KL divergence between two distributions $P$ and $R$ is 0, or almost as large as it could be (notice that if $R(x)/P(x)\le t\; \forall\; x \in \X$ then $\KL{R}{P} \le \log(t)$) needs a sample complexity polynomial in the size of the domain. The proof follows by a simple application of the birthday paradox, we note that it is possible to prove stronger lower bounds using better constructions \cite{BatuFRSW13,Valiant11} but we include the following result below for completeness.

\begin{lemma}\label{lem:impossibility}
\eat{
Let $P$ and $R$ be two distributions supported on some domain $\X$ of size $|\X|$. Say for any $t>0$ we are guaranteed that $R(x)/P(x)\le t\; \forall\; x \in \X$.  Then any algorithm for distinguishing whether $\KL{R}{P}=0$ or $\KL{R}{P} \ge \log(t)/10$ with success probability at least $2/3$ from i.i.d. samples from $P$ and $R$ requires at least $\Omega(\sqrt{|\X|})$ samples. }
Given any $t>0$ and a domain $\X$ of size $|\X|$, 
an  algorithm that, given two distributions $P,R$ over $X$ such that $R(x)/P(x) \le t$  can distinguish whether $\KL{R}{P}=0$ or $\KL{R}{P} \ge \log(t)/10$ with success probability at least $2/3$ from i.i.d. samples from $P$ and $R$, requires at least $\Omega(\sqrt{|\X|})$ samples.  
\end{lemma}
\begin{proof}
We first consider the case when $P$ and $R$ are both uniform distributions supported on half the domain (and the supports of both $P$ and $R$ are unknown to the algorithm). Note that by the birthday paradox, we not not expect to see any repetitions in $\sqrt{\X}/10$ samples drawn from a uniform distribution over a support of size $|\X|/2$, with probability $9/10$. Therefore, with $\sqrt{\X}/20$ samples drawn from $P$ and $R$, with probability $9/10$ we do not expect to any repetitions in the samples in either the case when $R=P$, or $R$ is a uniform distribution over a different support. Therefore no algorithm can distinguish between the case when $R=P$ or when the support of $R$ is drawn randomly and independently of $P$ with success probability more than $1/10$ given $O(\sqrt{\X})$ samples.

We can now leverage this lower bound to show a lower bound for any $t$ and some pair of distributions $R'$ and $P'$ such that $R'(x)/P'(x)\le t\; \forall\; x \in \X$. Let $U$ be the  uniform distribution over $\X$. For $P$ and $R$ as defined in the previous paragraph, let $P'=(2/t)U+(1-2/t)P$ and $R'=(2/t)U+(1-2/t)R$. Notice that in this case $R'(x)/P'(x)\in \{1,t-1\}\; \forall\; x \in \X \implies R'(x)/P'(x) \le t\; \forall\; x \in \X$. We note that if the support  of $R$ is chosen randomly and independently of the support of $P$, then by a Chernoff bound with probability $9/10$ the overlap in their supports is at most $|\X|/3$, which implies that $\KL{R'}{P'}\ge \log(t)/10$ with probability $9/10$. We now observe that if there exists an algorithm to distinguish whether $\KL{R'}{P'}=0$ or $\KL{R'}{P'} \ge \log(t)/10$ with success probability at least $p$ with $O(\sqrt{\X})$ samples, then it can be used to distinguish whether $R=P$ or $R$ is a uniform distribution over a different support as in the previous setup with success probability at least $(p-1/10)$ with $O(\sqrt{\X})$ samples. To verify this, observe that it is easy to generate $m$ samples from $P'$ and $R'$ given $m$ samples from $P$ and $R$. Therefore, by the lower bound in the previous paragraph, no algorithm can distinguish whether $\KL{R'}{P'}=0$ or $\KL{R'}{P'} \ge \log(t)/10$ with success probability at least $2/3$ with $O(\sqrt{\X})$ samples.

\end{proof}

\begin{proof}[Proof of Lemma \ref{lem:eq-est}]
The first estimator equals the LHS of (2) by definition (Equation \eqref{eq:est1}),  whereas the second equals the RHS of (2) by Equation \eqref{eq:est2.1}. The equivalence of (1) and (3) follows by equating the RHS of Equations \eqref{eq:est1} and \eqref{eq:est2}.
\end{proof}


\subsection{Proofs from Section \ref{sec:defs}}

\begin{proof}[Proof of Lemma \ref{lem:partition}]
    Note that for every $i \in [m]$, 
    \[ Q(S_i) = \sum_{x \in S_i} P(x)w(S_i) = P(S_i) \frac{R(S_i)}{P(S_i)}  = R(S_i).\]
    Under $Q$ every $x \in S_i$, has the same importance weight $w(S_i)$ relative to $P$, hence the conditional distributions $Q|_{S_i}$ and $P|_{S_i}$ are identical. 
\end{proof}

\subsection{Claims and Proofs from Section \ref{sec:mcab}}

\begin{lemma}
\label{lem:exp-close}
    $Q$ is $\alpha$-\mact for $(R, \mC)$. 
\end{lemma}
\begin{proof}
Using items (1) and (2) of Lemma \ref{lem:partition}, we can write
\begin{align*}
    Q(C) = \sum_{i \in [m]} R(S_i)P|_{S_i}(C) = \E_{\s \sim R}[P|_{\s}(C)], \    R(C) = \E_{\s \sim R}[R|_{\s}(C)]
\end{align*} 
Hence 
\begin{align*}
    \abs{Q(C) - R(C)} &= \abs{\E_{\s \sim R}[P|_{\s}(C)- R|_\s(C)]} \leq \E_{\s \sim R}\lt[\abs{P|_{\s}(C) - R|_\s(C)}\rt] \leq \alpha.
\end{align*}
\end{proof}



\begin{proof}[Proof of Lemma \ref{lem:stat}]
    By Lemma \ref{lem:partition} we have 
    \[ Q(S_i \cap C) = R(S_i) P|_{S_i}(C), \ \ R(S_i \cap C) = R(S_i)R|_{S_i}(C).\] 
    Hence
    \begin{align*}
     \lt|\frac{Q(S_i \cap C)}{Q(C)} -  \frac{R(S_i \cap C)}{R(C)}\rt|   &= R(S_i)\left|\frac{P|_{S_i}(C)}{Q(C)} - \frac{R|_{S_i}(C)}{R(C)} \right|\\
        & \leq \frac{R(S_i)}{R(C)}\abs{P|_{S_i}(C) - R|_{S_i}(C)} + R(S_i)P|_{S_i}(C)\left|\frac{1}{Q(C)} - \frac{1}{R(C)}\right|\\
        & \leq \frac{R(S_i)}{R(C)}\abs{P|_{S_i}(C) - R|_{S_i}(C)} +
        Q(S_i \cap C)\frac{\alpha}{Q(C)R(C)}
    \end{align*}
    where we use $|Q(C) - R(C)| \leq \alpha$ by Lemma \ref{lem:exp-close}. 
    We use this to bound the LHS of Equation \eqref{eq:sd} as
    \begin{align*}
             \lt|\sum_{i \in [m]}Q|_C(S_i) - R|_C(S_i) \rt| &\leq  \sum_{i \in [m]} \lt|\frac{Q(S_i \cap C)}{Q(C)} -  \frac{R(S_i \cap C)}{R(C)}\rt|\\
            & \leq \sum_{i \in [m]}\frac{R(S_i)}{R(C)}\abs{P|_{S_i}(C) - R|_{S_i}(C)} + \sum_{i \in [m]} Q(S_i \cap C)\frac{\alpha}{Q(C)R(C)}\\
            & \leq \frac{\alpha}{R(C)} + Q(C)\frac{\alpha}{Q(C)R(C)} = \frac{2\alpha}{R(C)}.
    \end{align*}
where the last line uses the definition of \mcbn.
\end{proof}


\begin{proof}[Proof of Lemma \ref{lem:pyth}]
By Equations \eqref{eq:est2} and \eqref{eq:est2.1} 
\begin{align*}
    \KL{R|_C}{P|_C} - \KL{R|_C}{Q|_C} &=  
    \E_{\s \sim R|_C}[\log(w(\s))] + \logf{P(C)}{Q(C)}  \\
\end{align*}
By Equation \eqref{eq:est1}
\begin{align*}
    \KL{Q|_C}{P|_C} &= \E_{\x \sim Q|_C} \left[ \logf{Q|_C(\x)}{P|_C(\x)}\right] = \E_{\s \sim Q|_C}[\log(w(\s))] + \logf{P(C)}{Q(C)}
\end{align*}
    Subtracting we get 
    \begin{align*}
    \abs{\KL{R|_C}{P|_C} - \KL{R|_C}{Q|_C} - \KL{Q|_C}{P|_C}} &=\abs{\E_{\s \sim R|_C}[\log(w(\s)] - \E_{\s \sim Q|_C}[\log(w(\s)]} \\
    & \leq \lt|\sum_{i \in [m]}R|_C(S_i) - Q|_C(S_i) \rt|\max_{i \in [m]}|\log(w(S_i))|\\
    &\leq 2\alpha\frac{\log(\infnorm{w})}{R(C)}.
    \end{align*}
    where we use the $(1, \infty)$ version of Holder's inequality, and then Lemma \ref{lem:stat}.
\end{proof}


\begin{proof}[Proof of Corollary \ref{cor:sandwich}]
We start by relating the central quantity to conditional KL divergence. For $x \in C$,
\begin{align*}
    w(x) = \frac{Q(x)}{P(x)}  = \frac{Q|_C(x)}{P|_C(x)} \frac{Q(C)}{P(C)} 
\end{align*}
Hence 
\begin{align}
    \label{eq:to-kl}
    \E_{R|_C}[\log(w(\x))] &= \E_{R|_C}\logf{Q|_C(\x)}{P|_C(x)} + \logf{Q(C)}{P(C)}
\end{align}
We can upper bound this as
\begin{align*}
    \E_{R|_C}\lt[\logf{Q|_C(\x)}{P|_C(x)}\rt] &= \KL{R|_C}{P|_C} - \KL{R|_C}{Q|_C} \\
    & \leq \KL{R|_C}{P|_C}\\
    & = \E_{R|_C}[\log(w^*(x))] + \logf{P(C)}{R(C)}.
\end{align*}
Hence using this in Equation \eqref{eq:to-kl},
\begin{align}
\E_{R|_C}[\log(w(\x))] & \leq  \E_{R|_C}[\log(w^*(x))] +\logf{P(C)}{R(C)} + \logf{Q(C)}{P(C)} \notag \\
&= \E_{R|_C}[\log(w^*(x))] +\logf{Q(C)}{R(C)} \label{eq:ub-p1}
\end{align}
By multiaccuracy, $Q(C) \leq R(C) + \alpha$. Hence 
\begin{align}
    \logf{Q(C)}{R(C)} \leq \log\lt(1 + \frac{\alpha}{R(C)}\rt) \leq  \frac{\alpha}{R(C)}. \label{eq:ub-p2}
\end{align}
Plugging Equation \eqref{eq:ub-p2} into \eqref{eq:ub-p1} gives the upper bound.

To show the lower bound, we start from Equation \eqref{eq:to-kl}. We lower bound the first term using the Pythagorean property as 
\begin{align}
\E_{R|_C}\logf{Q|_C(\x)}{P|_C(x)} & = \KL{R|_C}{P|_C} - \KL{R|_C}{Q|_C}\notag\\
& \geq \KL{Q|_C}{P|_C} - \frac{\beta}{R(C)} \geq - \frac{\beta}{R(C)}\label{eq:lb-p1}
\end{align}
where the last inequality uses the non-negativity of KL divergence.
For the last  term, we use $Q(C) \geq R(C) - \alpha$ and the inequality $\log(1- x) \geq -x/(1-x)$ to get
\begin{align*}
 \logf{Q(C)}{R(C)} \geq \log\lt(1 - \frac{\alpha}{R(C)}\rt) \geq -\frac{\alpha}{R(C) - \alpha} 
\end{align*}
hence
\begin{align}
 \logf{Q(C)}{P(C)} = \logf{R(C)}{P(C)} + \logf{Q(C)}{R(C)}  \geq \logf{R(C)}{P(C)} -\frac{\alpha}{R(C) - \alpha} \label{eq:lb-p2}
\end{align}

Plugging Equations \eqref{eq:lb-p1} and \eqref{eq:lb-p2}  into Equation \eqref{eq:to-kl} gives the lower bound 
\begin{align*}
    \E_{R|_C}[\log(w(\x))] \geq \logf{R(C)}{P(C)} -\frac{\beta}{R(C)} -\frac{\alpha}{R(C) - \alpha}
\end{align*}
\end{proof}

\subsection{Proofs from Section \ref{sec:macc}}
\label{sec:gap}

In this section we prove Theorem \ref{thm:gap-1}.
\eat{
Our counterexample is similar to counterexamples in \cite{gopalan2021multicalibrated}, and works by starting with a small example on $\zo^2$ that shows some small constant gap, and then tensoring to amplify the gap. The tensoring is made possible by the following property of KL divergence.

\begin{lemma}
\label{lem:tensor}
    Let $P$ and $R$ be distributions, and $P^k$ and $R^k$ be their $k$-wise products on $\X^k$. Then $\KL{R^k}{P^k} = k\KL{R}{P}$.
\end{lemma}
}

\begin{proof}[Proof of Theorem \ref{thm:gap-1}]
Let $P$ be the uniform distribution on $\zo^2$. Let $R$ be the distribution where
\[ R(00) = 1/4, R(01) = 1/4, R(10) = 0, R(11) =1/2. \]
We denote the two coordinates $x_0, x_1$, and let $\mC$ consist of all subcubes of dimension $1$. Hence $\mC = \{x: x_i =a\}_{i \in \zo, a \in \zo}$. 

 The distribution $Q^0$ for $\alpha = 0$ is the product distribution which matches the marginal distributions on each coordinate: $Q^0(x_0 =1) = 1/2, Q^0(x_1 = 1) = 3/4$, and the coordinates are independent. The \macc\ constraints hold since 
 \[ Q(x_0 =1) = R(x_0 =1) =1/2\]
 \[ Q(x_1 = 1) = R(x_1 = 1) = 3/4 \] 
 and $Q^0$ is the maximum entropy distribution satisfying these constraints since the co-ordinates are independent. 
 
 Now consider the set $C =\{x_0 =0\}$. Let $B(p)$ denote the Bernoulli distribution with parameter $p$. It follows that $R|_C = P|_C = B(1/2)$, whereas $Q^0|_C = B(3/4)$. Hence 
 \[ \KL{R|_C}{P|_C} = 0, \KL{R|_C}{Q|_C} = \KL{Q|_C}{P|_C} = d(3/4, 1/2). \] 
 Assume that $Q$ satsifies $(\alpha,\beta)$ multi-group attribution, so that
 \begin{align*}
     2\cdot d(3/4, 1/2) = \abs{\KL{R|_C}{P|_C} - \KL{R|_C}{Q|_C} - \KL{Q|_C}{P|_C}} \leq \frac{\beta}{R(C)} 
 \end{align*}
 Since $R(C) =1/2$, this implies $\beta \geq d(3/4, 1/2)$ as desired.
 \end{proof}
 


==> future.tex <==
\iffalse

\paragraph{Societal impact and limitations.}

One of the motivations of this work is algorithmic fairness, and to mitigate disparities between sub-populations that should be treated similarly. By now it is well understood that there are tradeoffs between different notions of fairness, and the right definitions to be deployed are context-dependent and depend on societal norms. This is doubly true for a framework like ours, where a family of definitions is suggested parameterized by the collection $\mathcal{C}$. We do not give guidance about what choice of $\mathcal{C}$ is most suitable, it depends on the context. We believe that exploring the landscape of definitions and guarantees is  critical even at the risk of abuse (a risk that exists for every work in this area).

\fi

==> old/app-def.tex <==
\section{Proofs}

\subsection{Proof of Theorem \ref{thm:p-to-cs}}
\label{app:cont}

\begin{proof}[Proof of Theorem \ref{thm:p-to-cs}]
We start by observing that since $Q(C) = R(C)$,
\begin{align*}
    w(x) &= \frac{Q(x)}{P(x)}  = \frac{Q|_C(x)}{P|_C(x)} \frac{R(C)}{P(C)}\\
    w^*(x) &= \frac{R(x)}{P(x)}  = \frac{R|_C(x)}{P|_C(x)} \frac{R(C)}{P(C)}
\end{align*}
Hence 
\begin{align*}
    \E_{R|_C}[\log(w(\x))]    &= \E_{R|_C}\lt[ \logf{Q|_C(\x)}{P|_C(x)} \rt] + \logf{Q(C)}{P(C)}\\
    & \leq \KL{R|_C}{P|_C}  + \logf{R(C)}{P(C)}\\
    & = \E_{R|_C}[\log(w^*(x)]
\end{align*}
where the inequality uses Lemma \ref{lem:lb}.

For the lower bound, we have 
\begin{align*}
    \E_{R|_C}[\log(w(\x))]    &= \E_{R|_C}\lt[ \logf{Q|_C(\x)}{P|_C(x)} \rt] + \logf{Q(C)}{P(C)}\\
    &=  \KL{R|_C}{P|_C} - \KL{R|_C}{Q|_C} +   \logf{R(C)}{P(C)}\\ 
    &= \KL{Q|_C}{P|_C} +   \logf{R(C)}{P(C)}  \geq \logf{R(C)}{P(C)} 
\end{align*}
\end{proof}


\subsection{Proofs from Section \ref{sec:lower}}
\label{app:intro}

We start by proving Lemma \ref{lem:lb}. 

\begin{proof}[Proof of Lemma \ref{lem:lb}]
    We have
    \begin{align*}
        \KL{R}{P} - \KL{R}{Q} &= \E_{\x \sim R}\left[\logf{R(\x)}{P(\x)}\right] - \left[\logf{R(\x)}{Q(\x)}\right]\\
        &= \E_{\x \sim R}\left[\logf{Q(\x)}{P(\x)}\right] = \E_{\x \sim R}[\log(w(\x))].
    \end{align*}
    The inequality follows from the non-negativity of KL divergence. 
\end{proof}

Lemma \ref{lem:lb} is essentially equivalent to the following bound from \cite{nguyen2010estimating}.  \cite{nguyen2007nonparametric} derive it using Fenchel duality. Below we give a somewhat simpler derivation of their proof. 

\begin{lemma}
 \cite[Equation 8]{nguyen2010estimating} 
\label{lem:nwj}
  Let $w: \X \rgta \R^+$. Then
  \begin{align}
    \label{eq:njw}
    \KL{R}{P} \geq \E_{R}[\log(w(\x))]  - \E_{P}[w(\x)] + 1. 
  \end{align}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:nwj}]
  We first claim that for all $y \in \R^+$,
  \begin{align}
  \label{eq:fenchel}
      \log(1/y) = \max_{t \geq 0} \log(t)- ty +  1.
  \end{align}
  The function $g(t) = \log(t) + 1 - ty$ is concave on $\R^+$ and is maximized when $g'(t) = 1/t- y = 0$. At $t = 1/y$ it takes the value $\log(1/y)$.

  Define the function $y(x) = P(x)/R(x)$. Using Equation \eqref{eq:fenchel}, for any $w: \X \rgta \R^+$ we have
  \begin{align*}
    \KL{R}{P}  &= \E_{R}[\log(1/y(\x))] \geq \E_{R}[\log(w(\x) - w(\x)y(\x) + 1 ]\\
    & = \E_R[\log(w(\x))] - \E_{R}\lt[\frac{w(\x)P(\x)}{R(\x)}\rt]  + 1 = \E_R[\log(w(\x))] - \E_{P}[w(\x)]  + 1.
  \end{align*}
\end{proof}


When $w(x) = Q(x)/P(x)$ is the importance weight of a distribution, $\E_{P}[w(\x)] =1$ and this reduces to Equation \eqref{eq:lb}. Conversely Equation \eqref{eq:njw} can be derived by replacing $\KL{R}{P}$ with the un-normalized KL divergence in the proof of Lemma \ref{lem:lb}. 


==> old/checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
\iffalse

The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section }
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\fi

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}, in Section \ref{sec:related}.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}, in Section \ref{sec:related}.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
     \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
     \answerYes{}
	\item Did you include complete proofs of all theoretical results?
     \answerYes{}, included in the Appendix.
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}, included in the supplementary material.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}, included in the Appendix and in the code in the supplementary material.
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}, we report it for our mixture of Gaussians experiment which uses a random seed to sample the data.
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}, included in the Appendix.
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> old/defs.tex <==
\section{Lower bounds on KL divergence}
\label{sec:lower}

Given two distribution $P, R$ on domain $\X$, our goal is to estimate the KL divergence between them. For a distribution $Q$ on $\X$, with importance weights $w$ relative to $P$,  we use the notation $Q = w \cdot P$ to denote this. We say the weights are explicit, if the function $w:\X \rgta \R$ is computable (efficiently). Note that  this does not necessarily require the pdf of $Q$ to be explicit.  We let  $R = w^*\cdot P$.  For a subset $C \subseteq \X$ and distribution $T$ on $\X$, recall the notation $T(C) = \Pr_{T}[\x \in C]$, and let $T|_C$ denote  distribution $T$ conditioned on the set $C$, so that $T|_C(x) = T(x)/T(C)$. We work with discrete distributions for simplicity, but one can have analogous definitions in the continuous setting.

The following lemma (proved in Section \ref{app:intro}) shows that any distribution whose importance weights $w$ relative to $P$ are explicit can be used to lower bound $\KL{R}{P}$ by estimating $\E_R[\log(w(\x))]$. 

\begin{lemma}
\label{lem:lb}
    For distributions $Q = w \cdot P$ and $R = w^*\cdot P$ on $\X$, we have
    \begin{align}
    \label{eq:lb}
    \KL{R}{P} - \KL{R}{Q}  = \E_{\x \sim R} [\log(w(\x))] \leq \E_{\x \sim R} [\log(w^*(\x))] = \KL{R}{P}.
    \end{align}
\end{lemma}

Versions of this lemma appear in \cite{KLIEP} in the context of density-ratio estimation, and \cite{nguyen2010estimating} in the context of divergence estimation. In the KLIEP algorithm of Sugiyama \etal \cite{KLIEP}, \cite[Chapter 5]{sugiyamaBook}, the goal is to find $Q =w \cdot P$ which minimizes $\KL{R}{Q}$. They use Equation \eqref{eq:lb} to reduce this to maximizing $\E_R[\log(w(\x))]$.
Lemma \ref{lem:lb} is essentially equivalent to a bound  of Nguyen \etal \cite[Equation 8]{nguyen2010estimating} for entropy estimation, see Section \ref{app:intro}.


==> old/div-fair.tex <==
Given samples form a (prior) distribution $P$ and an observed distribution $R$, we want to understand and measure how and by how much they diverge form one another. A natural approach would be to measure the KL divergence $\KL{R}{P}$ between them. 

A common approach to divergence estimation is through density-ratio estimation or importance weights: we build a model $Q = w \cdot P$ for $R$ where $w: \X \rgta \R^+$ are the importance weights.  We  use the estimator
\begin{align}
\label{eq:est1}
    \E_R[\log(w(\x))]  = \E_R\left[\logf{Q(\x)}{P(\x)}\right] = \KL{R}{P} - \KL{R}{Q} 
\end{align} 
Since $\KL{R}{Q} \geq 0$ for every $Q$, this gives a lower bound on the true KL divergence $\KL{R}{P}$. Since we know that $\KL{R}{P}$ is non-negative, the estimate given by Equation \eqref{eq:est1} is meaningful only when 
\begin{equation}
\label{eq:closer0}
    \KL{R}{P} \geq \KL{R}{Q}.
\end{equation}
In summary, this first estimator is conservative, but could be meaningless (negative).

The same model $Q$ also gives rise to a related but different estimator for $\KL{R}{P}$. We view $Q$ as a model for $R$, and computing the divergence from $P$: 
\begin{align}
\label{eq:est2}
    \E_Q[\log(w(\x))] = \KL{Q}{P}
\end{align}
In contrast with the previous estimator, this estimator is always non-negative. It is not guaranteed to be a lower bound on the true divergence though, it might exaggerate the divergence. For it to be a lower bound requires
\begin{align}
\label{eq:cons0}
    \KL{R}{P} \geq \KL{Q}{P}.
\end{align}

Wouldn't it be nice to have a single estimator which is both non-negative, and guarantees a lower bound on $\KL{R}{P}$?

The key difference from the estimator in Equation \eqref{eq:est1} is that the expectation of $\log(w(\x))$ is taken over $Q$ rather than $R$. There is a natural necessary and sufficient condition under which the two estimators return identical estimates: that the so-called Pythagorean theorem
\[ \KL{R}{P} = \KL{R}{Q} + \KL{Q}{P} \]
is satisfied for $P, Q, R$. The proof is immediate from Equation \eqref{eq:est1} and \eqref{eq:est2}. When this happens, the two estimators are identical:
\[\E_R[\log(w(\x))] = \E_Q[\log(w(\x))] = \KL{Q}{P} \]
Further, this estimator is both non-negative and conservative:
\[ 0 \leq \KL{Q}{P} \leq \KL{R}{P} \]

We now consider the following generalization. Let $\mC$ be a (possibly infinite) collection of subsets of $\X$. Our goal is to accurately model the contribution of each set $C \in \mC$ to the divergence. We require a single model $Q$ such that for every $C \in \mC$, 
\begin{align} 
\label{eq:c-sandwich}
0 \leq \KL{Q|_C}{P|_C} \leq \KL{R|_C}{P|_C}. 
\end{align}
Thus for every subset $C$, we want the conditional distribution $Q|_C$ to give a KL divergence estimate for $\KL{R|_C}{P|_C}$ which is both non-negative and conservative. We know that in order to achieve this, it suffies that the Pythagorean theorem holds conditioned on $C$:
\begin{align}
\label{eq:pyth}
    \KL{R|_C}{P|_C} = \KL{R|_C}{Q|_C} + \KL{Q|_C}{P|_C}.
\end{align}

\eat{


\section{older}

Let $\mC$ be a (possibly infinite) collection of subsets of $\X$. Our goal is to accurately model the contribution of each set $C \in \mC$ to the divergence. How do we formulate this problem of getting a model that  simultaneously gives accurate guarantees for every sub-population? Under what conditions do the weights $w$ let us do this?

We propose imposing the following constraints  for every $C \in \mC$:
\begin{align}
    Q(C) &= R(C) \label{eq:macc}\\
    \KL{Q|_C}{P|_C} &\leq \KL{R|_C}{P|_C} \label{eq:cons}\\
    \KL{R|_C}{Q|_C} &\leq \KL{R|_C}{P|_C} \label{eq:closer}
\end{align}
The first constraint is the multiaccuracy constraint following \cite{gopalan2021multicalibrated}, a number of algorithms will guarantee this. The second constraint requires that our model does not overestimate the true divergence conditioned on any set $C$. It guarantees that if our model says the divergence between $Q$ and $P$ conditioned on $C$ is large, then so is the true divergence $\KL{R|_C}{P|_C}$. The third constraint asserts that conditioned on $C$, the model $Q$ is closer to $R$ than our prior $P$. If this constraint is violated, then it means that conditioned on $C$, our learned model $Q$ is {\em worse}\footnote{as measured by KL divergence} than simply using the prior $P$. Equation \eqref{eq:closer} guarantees  that estimate of the conditional KL divergence given by Equation \eqref{eq:est1} is non-negative.


Further motivation for imposing these constraints can be derived from the sandwiching bounds proposed by \cite{gopalan2021multicalibrated}. Motivated by considerations of multigroup fairness for importance weight estimation, they proposed that the importance weights $w$ should satisfy:
\begin{align}
\label{eq:grsw-sandwich}
    \frac{R(C)}{P(C)} \leq \E_{R|_C}[w(\x)] \leq  \E_{R|_C}[w^*(\x)]
\end{align}
In analogy, we could require the importance weights to satisfy
\begin{align}
\label{eq:log-sandwich}
    \logf{R(C}{P(C)} \leq \E_{R|_C}[\log(w(\x))] \leq  \E_{R|_C}[\log(w^*(\x))]
\end{align}
As in \cite{GRSW21} these bounds guarantee {\em completeness} and {\em soundness} for the $\log(w(\x))$:  if $R(C)/P(C)$ is large, then so is the average value of $log(w(\x))$ over the set $C$; and if $\log(w(\x))$ is large on average over $C$,  then so are the ground truth weights $\log(w^*(\x)$.  
While Equation \eqref{eq:log-sandwich} looks similar to Equation \eqref{eq:grsw-sandwich}, neither implies the other (since log is concave). We will show Equation \eqref{eq:log-sandwich} can be derived from the constraints that we propose. Indeed, assuming multiaccuracy (Equation \eqref{eq:macc}) Equation \eqref{eq:log-sandwich} can be rewritten as
\begin{align}
    0 \leq \KL{R|_C}{P|_C} - \KL{R|C}{Q|_C} \leq \KL{R|_C}{P|_C}
\end{align} 
The upper bound is true by the non-negativity of KL divergence (thus  multiaccuracy alone suffices to guarantee it). The lower bound is just Equation
\eqref{eq:cons}. 



Equations \eqref{eq:cons} and \eqref{eq:closer} can be replaced by a single stronger constraint, we require that the Pythagorean theorem holds conditioned on every subset $C \in \mC$.
This  implies both  Equations \eqref{eq:cons} and \eqref{eq:closer} by the non-negativity of KL divergence. Intuitively, it captures the condition that the model $Q|_C$ lies {\em between} $R|_C$ and $P|_C$ when conditioned on $C$ for every $C \in \mC$ simultaneously.


Here is a different rationale for why Pythagorean theorems are natural. Let us return to the problem of divergence estimation for $R$ from $P$. 




We show that multicalibration with respect to $\mC$ guarantees Pythagorean theorems for every $C \in \mC$. Hence the derived importance weights satisfy the sandwiching bounds stipulated in Equation \eqref{eq:log-sandwich}. If we consider the model $Q = w \cdot P$ for $R$ which is specified by these weights, then the conditional distributions satisfy Equations \eqref{eq:macc}, \eqref{eq:cons} and \eqref{eq:closer}.  

As we mentioned earlier, while the sandwiching bounds in Equation \eqref{eq:log-sandwich} are inspired by the sandwiching bounds proposed by \cite{gopalan2021multicalibrated}, there are some important differences between them. Neither implies the other. Indeed, the upper bound in Equation \eqref{eq:log-sandwich} holds under multiaccuracy alone, while the lower bound is shown to hold under multicalibration. In contrast, for Equation \eqref{eq:grsw-sandwich}, both directions require multicalibration, indeed \cite{gopalan2021multicalibrated} give counterexamples showing that neither direction can be derived from multiaccuracy. Similarly, working with logs lets us translate the bounds to clean statements about KL divergence, for which there is a rich toolbox from information theory. The formulation in terms of the weights themselves (Equation \eqref{eq:grsw-sandwich}) does not seem to connect with a formulation in terms of say the Renyi divergence.


}

==> old/gap_maxent.tex <==

\eat{

\begin{lemma}
\label{lem:gap-1}
There exist distribution $P, R$ on $\zo^2$, a collections of sets $\mC$ and $C \in \mC$ such that the \maxent\ algorithm run on $(P, R, \mC)$ with $\alpha =0$ returns a distribution $\qme$ such that
 \begin{align}
    \label{eq:p-simple2}
    \abs{\KL{R|_C}{P|_C} - \KL{R|_C}{\qme|_C} - \KL{\qme|_C}{P|_C}}  > 0.15.
\end{align}
\end{lemma}
\begin{proof}


 The distribution $\qme$ for $\alpha = 0$ is the product distribution which matches the marginal distributions on each coordinate: $\qme(x_0 =1) = \qme(x_1 =1) = 5/8$ and the coordinates are independent. The \macc\ constraints $\qme(x_0 =1) = R(x_0 =1)$ and $\qme(x_1 = 1) = R(x_1 = 1)$ are clearly satisfied, and $\qme$ is the maximum entropy distribution satisfying these constraints. 
 
 We consider the set $C = \{10, 11\} = \{x: x_0 = 1\}$. Note that $P|_C$ is uniform on $x_1 \in \zo$, whereas $R|_C(x_1 = 1) = 2/5$.  As stated above, $\qme|_C(x_1 = 1) = 5/8$. Then it follows that (all logarithms are base 2)
 \begin{align*}
    \KL{R|_C}{P|_C} < 0.03, \KL{R|_C}{\qme|_C} > 0.145, \KL{\qme|_C}{P|_C} > 0.045.
 \end{align*}
 hence 
 $$
 \abs{\KL{R|_C}{P|_C} - \KL{R|_C}{\qme|_C} - \KL{\qme|_C}{P|_C}}  > 0.15.
 $$
 \end{proof}
 
 Intuitively, in the example above, while $\qme$ assigns the right weight of $5/8$ to the set $C$, within $C$ the distribution of weight is misaligned with $R$, leading to low expected weight under $R|_C$. We now tensor this example to amplify the gap.
 
\begin{proof}[Proof of Theorem \ref{thm:gap-1}]
 We now consider the $k$-wise tensor of the instances constructed in Lemma \ref{lem:gap-1}. The domain is $\zo^{2k}$ where the coordinates are denoted $x_0, \ldots, x_{2k-1}$. We consider the pair of distributions $P_k =(P)^k$ which is uniform on $2k$ bits, $R_k = (R)^k$ which the product of $k$ independent copies of $R$ on the pairs $\{x_{2i}x_{2i+1}\}_{i=1}^{k-1}$. Let $\mC_k$ consist of all subcubes of dimension $k$ where we restrict one co-ordinate out of $x_{2i}, x_{2i +1}$ for $i \in \{0,\ldots, k-1\}$. One can verify that \maxent\  returns $\qme_k = (\qme)^k$ which is just the product distribution on $\zo^{2k}$ with $\Pr[x_i =1] = 5/8$ for every coordinate. 
 
We consider the set $C = \{x: x_{2i} = 1, i \in \{0, \ldots, k-1\}\}$. The crucial property of this set is that the conditional distributions $P_k|_C = (P|_C)^k$ and $R_k|_C = (R|_C)^k$ are also product distributions of the conditional distributions. We now observe that since the KL-divergence tensors, we can write,
\begin{gather*}
   \KL{R_k|_C}{P_k|_C} = \sum_{i=0}^{k-1} \KL{R|_C}{P|_C} = k\KL{R|_C}{P|_C} ,\\
   \KL{R_k|_C}{\qme_k|_C} = k\KL{R|_C}{P|_C},\\
   \KL{\qme_k|_C}{P_k|_C} = k\KL{R|_C}{P|_C}.
  \end{gather*}
  
  Therefore,
  \begin{gather*}
   \abs{\KL{R|_C}{P|_C} - \KL{R|_C}{\qme|_C} - \KL{\qme|_C}{P|_C}}  =  0.15k.
  \end{gather*}
  
  We can now take $k$ sufficiently large so that $0.15k > B$.
  \end{proof}
  

}

==> old/maxent.tex <==
\section{The \maxent algorithm}



\begin{definition}
Let $Q^\alpha$ to be the distribution from $K(R, \alpha)$ whose KL divergence from $P$ is the minimum. Thus $Q^\alpha$ is the unique optimal solution to the following strictly convex program
  \begin{equation}
  \label{eq:prog1}
      \begin{aligned}
        & \underset{Q \in K(R, \alpha)}{\text{minimize}} & & \KL{Q}{P}.
      \end{aligned}
    \end{equation}
\end{definition}

In the case when $P$ is the uniform distribution, this corresponds to finding $Q \in K(R, \alpha)$ that has maximum entropy. This problem was studied in the \maxent work of Dudik \etal who gave an elegant algorithm for it \cite{DudikPS04, Maxent}, by solving the Fenchel dual. Let $\mG(P, \mC)$ denote the set of all {\em Gibbs distributions} of the form
\begin{align}
    Q(x) &= P(x) \exp\left(\sum_{c \in \mC} \lambda_c c(x) -\lambda_0\right)  \label{eq:gibbs}\\
\text{where} \     \lambda_0 &= \log\lt(\E_{P}\lt[\exp\lt(\sum_{c \in \mC} \lambda_c c(x)\rt)\rt]\rt)\label{eq:gibbs2}
\end{align}
Note that the free parameters are $\lambda_\mC =\{\lambda_c\}_{c \in \mC}$.
As shown in \cite{DudikPS04}, for every $\alpha > 0$,  $Q^\alpha \in \mG(P, \mC)$. A standard property of Gibbs distributions that we will use is that they are uniquely defined by $\{\E_Q[c(\x)]\}_{c \in \mC}$.



We show that the \maxent algorithm arises naturally in our framework of KL estimation while using Gibbs distributions.  Gibbs distributions are natural for our framework, since the weight function $Q(x)/P(x)$ is explicit if we can evaluate functions in $\mC$ efficiently. Lemma \ref{lem:lb} when specialized to Gibbs distributions give the following lower bound.

\begin{lemma}
    For all $\lambda_\mC  \in \R^\mC$, we have
    \begin{align}
    \label{eq:gibbs-lb}
        \KL{R}{P} \geq f(\lambda_\mC) := \sum_{c \in \mC} \lambda_c\E_R[c(\x)] - \log\lt(\E_{P}\lt[\exp\lt(\sum_{c \in \mC} \lambda_c c(x)\rt)\rt] \rt)
    \end{align}
\end{lemma}
\begin{proof}
    Applying  Lemma \ref{lem:lb} gives the lower bound
    \begin{align*}
    \KL{R}{P} \geq \E_R\lt[\logf{Q(\x)}{P(\x)}\rt] = \E_R\lt[\sum_c \lambda_c c(\x) - \lambda_0\rt] = \sum_c \lambda_c\E_R[c(\x)] - \lambda_0 = f(\lambda_\mC). 
    \end{align*}
\end{proof}


It is natural to ask which Gibbs distribution, or equivalently what parameters $\lambda_\mC$ maximize $f(\lambda_\mC)$. This is where the connection to \maxent arises.

\begin{lemma}
    $Q^0$ maximizes the lower bound in Equation \eqref{eq:gibbs-lb} over all distributions in $\mG(P, \mC)$. 
\end{lemma}
\begin{proof}
From Equation \eqref{eq:gibbs2}, we can write
    \[ \frac{\partial \lambda_0}{\partial \lambda_c} = \frac{\partial 
    \log\lt(\E_{P}\lt[\exp\lt(\sum_{c \in \mC} \lambda_c c(x)\rt)\rt]\rt)}{\partial \lambda_c} = 
    \frac{\E_{P}\lt[c(\x)\exp\lt(\sum_{c \in \mC} \lambda_c c(\x)\rt)\rt]}{
    \E_{P}\lt[\exp\lt(\sum_{c \in \mC} \lambda_c c(\x)\rt)\rt]} = \E_Q[c(\x)] \]
    Hence for the derivative wrt to $\lambda_c$ to vanish we require
    \[ \frac{\partial f}{\partial \lambda_c} = \E_R[c(x)] - \frac{\partial \lambda_0}{\partial \lambda_c} = \E_R[c(\x)] - \E_Q[c(\x)] = 0\]
    Since $Q^0 \in K(R, 0)$, the gradient vanishes at $Q_0$. 
    Since Gibbs distributions are uniquely defined by $\{\E_Q[c(\x)]\}_{c \in \mC}$, $Q_0$ is in fact the unique minimizer for $f(\lambda)$. 
\end{proof}

Given sample access to $R$ and $P$, we cannot hope to compute $Q^0$, but there are efficient algorithms to find $Q^\alpha$ for small $\alpha$ \cite{dudik2007maximum}. Since $Q^\alpha$ minimizes $\KL{Q}{P}$ over $K(R, \alpha) \ni R$, we have
\begin{align}
\label{eq:trivial}
    \KL{R}{P} \geq \KL{Q^\alpha}{P} 
\end{align}
How does this bound compare with the bound obtained using Lemma \ref{lem:lb}? We can answer this question using the Pythagorean theorem for projections onto convex sets \cite[Theorem 11.6.1]{CT}, which when applied in this context gives
\begin{align}
    \KL{R}{P} - \KL{R}{Q^\alpha} \geq \KL{Q^\alpha}{P}.
\end{align}
Observe that the LHS is precisely our lower bound from Lemma \ref{lem:lb}, which is stronger. Indeed, we can quantify the gap between the two bounds exactly. For a Gibbs distribution as in Equation \eqref{eq:gibbs}. let $\ell_1(Q) = \sum_{c \in \mC}|\lambda_c|$.

\begin{theorem}
\label{thm:pyth}
    For any $\alpha > 0$ we have
    \begin{align}
    \label{eq:pyth}
        \KL{R}{P} - \KL{R}{Q^\alpha} = \KL{Q^\alpha}{P} + \alpha \ell_1(Q).
    \end{align}
\end{theorem}

This result shows a Pythagorean theorem for $R, P$ and $Q^\alpha$. It is natural to ask if a similar result holds even conditioned on the sets $C \in \mC$. We show a strong negative result, even for the case where $\alpha =0$. 

\begin{theorem}
\label{thm:gap-1}
For any constant $B > 1$, there exist distributions $P, R$ on $\zo^n$, a collections of sets $\mC$ and $C \in \mC$ such that distribution $Q^0$ returned by \maxent with $\alpha =0$ satisfies
\begin{align}
    \label{eq:p-simple2}
    \abs{\KL{R|_C}{P|_C} - \KL{R|_C}{Q^0|_C} - \KL{Q^0|_C}{P|_C}}  > B.
\end{align}
\end{theorem}



\eat{
Our first main result is showing that the following {\em Pythagorean} theorem holds:
\begin{theorem}
\label{thm:pyth}
  For any $\eps > 0$, we have
\begin{align}
  \label{eq:pyth}
  \kl(\rb, \pb)  &= \kl(\rb, \qb^\eps) + \kl(\qb^\epsilon, \pb) + \epsilon \ell_1(\qb^\eps)\\
  \label{eq:lb}
  \text{hence} \   \kl(\rb, \pb)  &\geq \kl(\qb^\epsilon, \pb) + \epsilon \ell_1(\qb^\eps).
\end{align}
\end{theorem}

Theorem \ref{thm:pyth} gives a convenient decomposition of the
$\kl(\rb, \pb)$.

\begin{tightenumerate}
   \item $\kl(\qb^\eps, \pb)$ is the $(\H, \eps)$-observed
     divergence, which lower bounds $\kl(\rb, \pb)$.
     Since $\kl(\qb^\eps, \pb) = \qb^\eps[\log(\qb^\eps/\pb)]$
   and the function $\log(\qb^\eps/\pb)$ is known to us explicitly,
   we can decompose it as a sum of contributions from  individual
   points $x$ in the domain.

 \item We refer to $\kl(\rb, \qb^\eps)$ as the {\em hidden divergence}
   since it is not known to us and it measures divergence between
   distributions that are near indistinguishable. Indeed $\kl(\rb,
   \qb^0)$ represents a fundamental limit in terms of divergence that cannot be measured
   using $\H$, regardless of the number of samples and
   computational power we invest.
   Similarly, $\kl(\rb, \qb^\eps)$ is hidden divergence that cannot be measured
   unless we increase the accuracy of our tests. In Theorem
   \ref{thm:error}, we will show that it gives tight bounds on the
   accuracy of the anomaly scores derived from $\qb^\eps$.


 \item The regularizer term $\eps \ell_1(\qb^\eps)$ represents a portion of
   $\kl(\rb, \pb)$ that lies in between hidden KL divergence and observed KL
   divergence. Unlike hidden divergence, we can measure it. But unlike
   observable divergence, we cannot (yet) allocate it to individual points in
   the domain. In Theorem \ref{thm:monotone}, we show that it lower
   bounds how much observed  divergence one can hope to gain by
   increasing the precision of our measurements. Intuitively,
   we can convert this into observed divergence with
   improved accuracy.
\end{tightenumerate}
Equation \eqref{eq:lb} presents a computable lower bound for the KL
divergence.  In practice, owing to computational and
sample constraints, it is hard to  drive $\eps$ down beyond a
point, hence this lower bound is useful.

Theorem \ref{thm:pyth} builds on the work of \cite{DudikPS04} and is proved
using convex duality and the KKT conditions on the optimal
solutions. The inequality   $\kl(\rb, \pb) \geq \kl(\rb, \qb^\eps) +
\kl(\qb^\epsilon, \pb)$ is known, indeed a similar
bound holds for projection onto any convex polytope \cite[Chapter
  12]{CoverT}. Equation \eqref{eq:lb} is new, and gives a
computable lower bound on the KL divergence.
When $\eps =0$, the bound $\kl(\rb, \pb) = \kl(\rb,
\qb^0) +  \kl(\qb^0, \pb)$, is proved in the work of
\cite{PietraPL97}.
}

==> old/nwj.tex <==
\section{The \cite{nguyen2007nonparametric} approach}


\section{The \maxent algorithm}




\eat{
Let $\H = \{h: \Dc \rgta [-1,1]\}$ be a class of distinguishers. Let
  us consider all functions of the form
  \[ t(x) = \exp(\sum_{i \in \H} \lambda_h h(x) - \lambda_0) \]
  where $\lambda_h$ for $h \in \H$ are unrestricted and $\lambda_0$ is
  a renormalization constant chosen such that
  \[\E_\pb[t(x)] = 1.\]
  Note that for this choice of $t(x)$, the function
  \[q(x) \defeq t(x)p(x) = p(x)\exp(\sum_{i \in \H} \lambda_h h(x) - \lambda_0) \]
  is a Gibbs distribution. For this choice of $t(x)$, Corollary
  \ref{cor:one} yields the lower bound
    \begin{align*}
      \kl(\rb, \pb) & \geq \rb[\log(t)]  - \pb[t] + 1 = \sum_{i \in \H}\lambda_h\rb[h] - \lambda_0
    \end{align*}
    One can interpret this lower bound as follows
    \begin{align*}
      \sum_{i \in \H} \lambda_h \rb[h] - \lambda_0
          &= \E_{\rb}[\exp(\sum_{i \in \H} \lambda_h h(x) - \lambda_0)]\\
      &=          \E_{\rb}[\log(\qb(x)/\pb(x))]\\
          &=           \kl(\rb, \pb) - \kl(\rb, \qb).
    \end{align*}
}

==> old/pyth-proof.tex <==
\subsection{Proofs from Section \ref{sec:macc}}
\label{app:macc}

\eat{
\begin{lemma}
\label{lem:dual}
\cite{dudik2007maximum}
$Q^\alpha$ is the optimal solution to the following program:
  \begin{equation}
  \label{eq:prog2}
  \begin{aligned}
    & \underset{Q \in \mG(P, \mC)}{\text{minimize}} & & \KL{R}{Q} +
    \alpha \ell_1(Q).
  \end{aligned}
  \end{equation}
 \end{lemma}
  
The case $\alpha =0$ is treated in the work of Della Pietra \etal  \cite{PietraPL97}. 

}


\subsubsection{Pythagorean theorem for $Q^\alpha$}


\begin{theorem}
\label{thm:pyth}
    For any $\alpha > 0$ we have
    \begin{align}
    \label{eq:pyth-exact2}
        \KL{R}{P} = \KL{R}{Q^\alpha} + \KL{Q^\alpha}{P} + \alpha \ell_1(Q^\alpha).
    \end{align}
\end{theorem}

We start by proving a technical lemma relating the primal and dual
formulations given by Programs \eqref{eq:primal} and
\eqref{eq:dual}. For technical reasons, it will be useful to consider
a generalization where for each $c \in \mC$, we have a different error
parameter $\alpha_c$. Hence the primal program is

  \begin{equation}
  \label{eq:prog1.1}
  \begin{aligned}
    {\text{minimize}}  \KL{Q}{P}\\
    s.t. \forall c \in \mC, \ \lt|\E_R[c(x)] - \E_Q[c(x)]\rt|  \leq \alpha_c
  \end{aligned}
  \end{equation}
  whereas the dual program is
  \begin{equation}
  \label{eq:prog2.1}
  \begin{aligned}
    & \underset{Q \in \mG(P)}{\text{minimize}} & & \KL{R}{Q} +
    \sum_{c \in \mC}\alpha_c |\lambda_c|.
  \end{aligned}
  \end{equation}


  The following lemma is implicit in the work of \cite{KazamaT, dudik2007maximum}, and essentially states the Karush-Kuhn-Tucker conditions for optimality. we provide a proof for completeness.

  \begin{lemma}
    \label{lem:main_tech}
  The Gibbs distribution $Q(x)$ with parameters $\lambda_\mC$
  is optimal for  programs  \eqref{eq:prog1.1} and \eqref{eq:prog2.1} iff
  \begin{align}
    \label{eq:ineq}
    \forall c \in \mC, \ \lt| \E_R[c(x)] - \E_Q[c(x)] \rt|  &\leq \alpha_c,\\
    \label{eq:sign}
    \forall h: \lambda_c \neq 0, \ E_R[c(x)] - E_Q[c(x)]  & = \alpha_c\sign(\lambda_c).
  \end{align}
  \end{lemma}
  \begin{proof}
  Let $Q(x)$ be as in Equation \eqref{eq:gibbs}. Recall that the free
  variables in defining $Q$ are $\lambda_\mC$ from which we get
  \begin{align}
    \lambda_0 & = \log\left(\E_{P}\left[ \exp\left(\sum_{c \in \mC}
    \lambda_c c(x)\right)\right]\right).\label{eq:partition}\\
    \frac{\partial \lambda_0}{\partial \lambda_c} &=
    \frac{\E_{P}\left[c(x) \exp\left(\sum_{c \in \mC} \lambda_c
        c(x)\right)\right]}{\E_{P}\left[\exp\left(\sum_{c \in \mC}
    \lambda_c c(x)\right)\right] } = E_Q[c(x)].\label{eq:partial1}
  \end{align}
  Let $g(\lambda) = \KL{R}{Q} + \sum_h \alpha_c |\lambda_c|$ denote the objective
  function of Program \eqref{eq:prog2.1}. Then
  \begin{align*}
    g(\lambda) &= \KL{R}{P} + \E_R[\logf{P(\x}{Q(\x)}] + \sum_c \alpha_c |\lambda_c|\notag\\
    & = \KL{R}{P}  + \lambda_0 - \sum_h \lambda_c E_R[c(x)] + \sum_h
    \alpha_c|\lambda_c|
    \end{align*}
  Let $\frac{\partial g}{\partial \lambda_c}$ denote the
  family of subgradients and $\sign(0) = [-1, 1]$, we have
  \begin{align}
  \frac{\partial g}{\partial \lambda_c} = \frac{\partial
    \lambda_0}{\partial \lambda_c} - \E_R[c(\x)] + \alpha_c\sign(\lambda_c) =
  \E_Q[c(\x)] - \E_R[c(\x)] + \alpha_c \sign(\lambda_c). \label{eq:partial2}
  \end{align}
  Note that $\lambda$ is a minimizer of $g$ iff $0^\mC \in \nabla g$.
  It is easy to check that $0 \in \frac{\partial g}{\partial
    \lambda_c}$ iff Equations \eqref{eq:ineq} and \eqref{eq:sign} hold.
\end{proof}




We will formulate and prove the following generalization of
Theorem \ref{thm:pyth}, which allows for the general form of
Programs \eqref{eq:prog1.1} and \eqref{eq:prog2.1}.


\begin{theorem}
\label{thm:pyth_ext}
  If the Gibbs distribution $Q^*(x)$ with parameters $\{\lambda^*_c\}_{c \in \mC}$
  is optimal for  programs  \eqref{eq:prog1.1} and \eqref{eq:prog2.1}, then
  \[ \KL{R}{P} = \KL{R}{Q^*} + \KL{Q^*}{P} + \sum_c \alpha_c|\lambda^*_c|. \]
\end{theorem}
\begin{proof}
  By Lemma \ref{lem:main_tech},  for $c: \lambda^*_c \neq   0$,
  \begin{align}
    \label{eq:kkt}
    E_R[c(x)]  = Q^*[h] +  \alpha_c\sign(\lambda^*_c)
  \end{align}
We use this to prove Theorem \ref{thm:pyth_ext}.
  Note that without loss of generality, we can restrict the sum
  $\sum_c \lambda^*_c c(x)$ in the definition of $Q^*$ to only
  those where $\lambda_c \neq 0$, and for these Equation
  \eqref{eq:kkt} holds.  Hence have
  \begin{align*}
    \KL{R}{P} - \KL{R}{Q^*} 
      &= \E_R\left[\sum_{c\in  \mC} \lambda^*_cc(x) -
        \lambda^*_0\right]\\
      &= \lt(\sum_{c}\lambda^*_c\E_R[c(x)] - \lambda^*_0\rt)\\
      &= \lt(\sum_{h}\lambda^*_c(\E_Q[c(x)] + \alpha_c
    \sign(\lambda^*_c)) - \lambda^*_0\rt) \hspace{1cm} \text{by
      Equation \eqref{eq:kkt}}\\
      &= \lt(\sum_c\lambda^*_c\E_Q[c(x)] -\lambda^*_0\rt) +
      \sum_{h}\alpha_c|\lambda^*_c|\\
      &= Q^*\left[\sum_{c \in \mC} \lambda^*_cc(x) - \lambda^*_0\right]
      + \sum_c \alpha_c|\lambda^*_c|\\
      &= \E_{Q^*}[\logf{Q^*(\x)}{P(\x)}] + \sum_c \alpha_c|\lambda^*_c|\\
      &= \KL{Q^*}{P} + \sum_c \alpha_c|\lambda^*_c|
  \end{align*}
  \end{proof}


